Modelling the 3D spatiotemporal organisation of chromatin replication

We propose a polymer model for the dynamics of chromatin replication in three dimensional space. Our simulations indicate that both immobile and tracking replisomes may self-assemble during the process, reconciling previous apparently discordant experimental evidence in favour of either scenario. Which of the two morphologies appears in our model depends on the balance between non-specific and origin-targeting interactions between chromatin and firing factors -- polymerases and other components of the replisome. Non-specific interactions are also necessary to yield clustering of factors and replication forks, creating structures akin to the replication foci observed in mammalian cells in vivo. We suggest that cluster formation provides an underappreciated but robust pathway to avoid stalled or faulty forks, which would otherwise diminish the efficiency of the replication process. Additionally, our simulations allow us to predict different modes of cluster growth during S-phase, which could be tested experimentally, and they show that the three dimensional chromatin context is important to understand replication patterns in fission yeast.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


